Generalized classical Yang-Baxter equation and regular decompositions

The focus of the paper is on constructing new solutions of the generalized classical Yang-Baxter equation (GCYBE) that are not skew-symmetric. Using regular decompositions of finite-dimensional simple Lie algebras, we construct Lie algebra decompositions of $\mathfrak{g}(\!(x)\!) \times \mathfrak{g}[x]/x^m \mathfrak{g}[x]$. The latter decompositions are in bijection with the solutions to the GCYBE. Under appropriate regularity conditions, we obtain a partial classification of such solutions. The paper is concluded with the presentations of the Gaudin-type models associated to these solutions.

==> settings.tex <==
%% For formatting the tables
\usepackage{array}

%% Geometry of the page
\RequirePackage[margin=2.5cm]{geometry}

%% Pictures and figures
\usepackage{graphicx}
\usepackage{svg}
\usepackage{float} % to use H option
\usepackage{pdfpages} % to insert pdfs

%% Font encodings
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}

%% Bibliography
\usepackage[
backend=bibtex,
style=numeric,
maxbibnames=99,
maxcitenames = 99
]{biblatex}
\addbibresource{bibliography.bib}

%% For table of symbols
\usepackage{adjustbox}
\usepackage{hhline} % for the double line in table
\usepackage{makecell} % allows to wrap text in tables into cells
\usepackage{caption} % to make caption without :

%%%%%%%%%%%%%%%%%%%%%%%%
%Show refrences in equations
%\usepackage[ignoreunlbld]{refcheck}

%%%%%%%%%%%%%%% MATH (and references) %%%%%%%%%%%%%%%
%% Math packages
\usepackage{amsmath, amsthm, amssymb}
\usepackage{mathtools}

%for upside down widehat
%% code from mathabx.sty and mathabx.dcl
\DeclareFontFamily{U}{mathx}{\hyphenchar\font45}
\DeclareFontShape{U}{mathx}{m}{n}{
      <5> <6> <7> <8> <9> <10>
      <10.95> <12> <14.4> <17.28> <20.74> <24.88>
      mathx10
      }{}
\DeclareSymbolFont{mathx}{U}{mathx}{m}{n}
\DeclareFontSubstitution{U}{mathx}{m}{n}
\DeclareMathAccent{\widecheck}{0}{mathx}{"71}

%% References
\usepackage{nameref}
\usepackage{hyperref}
% \hypersetup{colorlinks,
%   linkcolor=ThesisDarkBlue,
%   citecolor=ThesisPurple,
%   urlcolor=ThesisDarkBlue,
%   filecolor=ThesisDarkBlue}
\usepackage[capitalise, nameinlink]{cleveref} % has to be added after amsmath
\newcommand{\crefrangeconjunction}{--}

%% QED symbol = black square
\renewcommand{\qedsymbol}{\ensuremath{\blacksquare}}

%% Mathfrak
\newcommand{\fg}[0]{\mathfrak{g}}
\newcommand{\fl}[0]{\mathfrak{l}}
\newcommand{\fp}[0]{\mathfrak{p}}
\newcommand{\fs}[0]{\mathfrak{s}}
\newcommand{\ft}[0]{\mathfrak{t}}
\newcommand{\fr}[0]{\mathfrak{r}}
\newcommand{\fc}[0]{\mathfrak{c}}
\newcommand{\fM}[0]{\mathfrak{M}}
\newcommand{\fn}{\mathfrak{n}}
\newcommand{\fh}{\mathfrak{h}}
\newcommand{\fb}[0]{\mathfrak{b}}
\newcommand{\fT}{\mathfrak{T}}
\newcommand{\fD}{\mathfrak{D}}

%% Killing form
\newcommand{\kf}{\kappa}

%% Mathbb
\newcommand{\bC}[0]{\mathbb{C}}
\newcommand{\bN}[0]{\mathbb{N}}
\newcommand{\bZ}[0]{\mathbb{Z}}
\newcommand{\bR}[0]{\mathbb{R}}

%% Operators
\newcommand{\add}{\dotplus}
\newcommand{\ot}{\otimes}
\newcommand{\op}{\oplus}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\colim}{colim}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\ad}{ad}

%%
\renewcommand{\ge}{\geqslant}
\renewcommand{\le}{\leqslant}

%%%%%%%%%%% ENVIRONMENTS %%%%%%%%%%%%%%%%
\newtheorem{thm}{Theorem}[section]
\theoremstyle{plain}

\newtheorem{maintheoremcounter}{maintheoremcounter}
\newtheorem{maincorollary}[maintheoremcounter]{Corollary}
\newtheorem{maintheorem}[maintheoremcounter]{Theorem}
\renewcommand{\themaintheoremcounter}{\Alph{maintheoremcounter}}

\newtheorem{corollary}[thm]{Corollary}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{proposition}[thm]{Proposition}
\newtheorem{theorem}[thm]{Theorem}
\newtheorem{conjecture}[thm]{Conjecture}

\theoremstyle{definition}
\newtheorem{definitionx}[thm]{Definition}
\newenvironment{definition}
  {\pushQED{\qed}\renewcommand{\qedsymbol}{$\lozenge$}\definitionx}
 {\popQED\enddefinitionx}

% Example/Remark style
\newtheoremstyle{example_style}
  {10pt} % Space above
  {10pt} % Space below
  {} % Body font
  {} % Indent amount
  {\itshape} % Theorem head font
  {.} % Punctuation after theorem head
  {10pt} % Space after theorem head
  {} % Theorem head spec (can be left empty, meaning `normal')

\theoremstyle{example_style}
% examplex is wrapped into example, which just adds lozenge at the end
\newtheorem{examplex}[thm]{Example}
\newenvironment{example}
  {\pushQED{\qed}\renewcommand{\qedsymbol}{$\lozenge$}\examplex}
  {\popQED\endexamplex}

\crefname{examplex}{Example}{Examples} % Name for cleverref

% Similarly with remark
\newtheorem{remarkx}[thm]{Remark}
\newenvironment{remark}
  {\pushQED{\qed}\renewcommand{\qedsymbol}{$\lozenge$}\remarkx}
 {\popQED\endremarkx}

